Evidence for evolving Dark Energy from a new cosmic probe

The $\Lambda$CDM concordance cosmological model provides a remarkably successful description of the formation and evolution of structure in the Universe. However, a growing discrepancy between measurements of the expansion rate $H_0$ from the near and distant Universe now appears to be significant at the ~4-7 $\sigma$ level. This inconsistency, known as the ``Hubble tension'', has arisen either due to unrecognized systematics in these measurements or new physics beyond the standard model, such as an evolving dark energy equation of state. Modeling ~20-year, multi-band optical light curves for 6992 active galactic nuclei (AGN), we find a tight relation linking the variability amplitude and characteristic timescale to their intrinsic luminosity. This empirical law enables us to construct an AGN-based Hubble diagram to z ~3.5. Joint inference with supernova distances reveals evidence for an evolving dark energy equation of state at the 3.8-3.9 $\sigma$ level over constant w models and 4.4-4.8 $\sigma$ over $\Lambda$CDM. Our results establish AGN light curves as a powerful tool for cosmography that could offer a novel pathway to test deviations from the standard $\Lambda$CDM expansion history.

==> agn_table.tex <==
\begin{tabular}{@{}lccccccccc@{}}
\hline\hline
\textbf{SDSS Name} & RA & Dec & $z$ & $m_{2500}$ & $m_{2500}^{\mathrm{uncorr}}$ & $\mu$ & $\log\tau_{\mathrm{UV,RF}}$ & $\log\sigma_{\mathrm{UV}}$ & $\mathrm{Cov}(\log\sigma_{\mathrm{UV}},\,\log\tau_{\mathrm{UV,RF}})$ \\
& (deg) & (deg) &  & (mag) & (mag) & (mag) & (days) & (mag) &  \\\hline
\textbf{J011307.50$-$002309.4} & $18.2813$ & $-0.3860$ & $0.4549 \pm 0.0004$ & $21.44 \pm 0.02$ & $22.19 \pm 0.02$ & $43.81 \pm 1.22$ & $2.98 \pm 0.34$ & $-0.67 \pm 0.17$ & $0.028$ \\
\textbf{J235645.71$-$010801.8} & $359.1905$ & $-1.1339$ & $0.6996 \pm 0.0005$ & $21.88 \pm 0.02$ & $21.92 \pm 0.02$ & $42.90 \pm 1.41$ & $2.48 \pm 0.67$ & $-0.58 \pm 0.12$ & $0.017$ \\
\textbf{J212252.87+010900.8} & $320.7203$ & $+1.1502$ & $0.9437 \pm 0.0010$ & $22.43 \pm 0.03$ & $21.84 \pm 0.03$ & $43.54 \pm 0.99$ & $3.50 \pm 0.26$ & $-0.34 \pm 0.14$ & $0.029$ \\
\textbf{J015859.25$-$000114.1} & $29.7469$ & $-0.0206$ & $1.0222 \pm 0.0005$ & $23.11 \pm 0.03$ & $22.50 \pm 0.03$ & $43.80 \pm 0.96$ & $2.50 \pm 0.31$ & $-0.52 \pm 0.11$ & $0.023$ \\
\textbf{J230332.16$-$004421.4} & $345.8840$ & $-0.7393$ & $1.0233 \pm 0.0005$ & $22.53 \pm 0.02$ & $22.14 \pm 0.02$ & $45.45 \pm 1.16$ & $2.78 \pm 0.45$ & $-0.81 \pm 0.17$ & $0.046$ \\
\textbf{J000901.84+001146.6} & $2.2577$ & $+0.1963$ & $1.0434 \pm 0.0020$ & $21.86 \pm 0.02$ & $21.50 \pm 0.02$ & $43.30 \pm 0.95$ & $2.85 \pm 0.28$ & $-0.56 \pm 0.12$ & $0.028$ \\
\textbf{J225937.63$-$004204.3} & $344.9068$ & $-0.7012$ & $1.0545 \pm 0.0024$ & $22.51 \pm 0.02$ & $21.94 \pm 0.02$ & $42.93 \pm 0.98$ & $2.89 \pm 0.25$ & $-0.39 \pm 0.11$ & $0.019$ \\
\textbf{J003410.01+011350.5} & $8.5417$ & $+1.2307$ & $1.0908 \pm 0.0020$ & $21.20 \pm 0.02$ & $21.11 \pm 0.02$ & $42.83 \pm 1.05$ & $3.48 \pm 0.26$ & $-0.43 \pm 0.15$ & $0.029$ \\
\textbf{J004730.03+003120.3} & $11.8751$ & $+0.5223$ & $1.1398 \pm 0.0022$ & $23.00 \pm 0.03$ & $22.38 \pm 0.03$ & $45.08 \pm 1.22$ & $3.29 \pm 0.38$ & $-0.55 \pm 0.17$ & $0.036$ \\
\textbf{J212331.51$-$001742.3} & $320.8813$ & $-0.2951$ & $1.1565 \pm 0.0009$ & $22.37 \pm 0.02$ & $21.79 \pm 0.02$ & $44.23 \pm 1.01$ & $3.18 \pm 0.35$ & $-0.54 \pm 0.16$ & $0.048$ \\
\textbf{J230926.24$-$001044.8} & $347.3594$ & $-0.1791$ & $1.1695 \pm 0.0009$ & $22.36 \pm 0.02$ & $21.78 \pm 0.02$ & $44.11 \pm 0.94$ & $2.68 \pm 0.21$ & $-0.65 \pm 0.09$ & $0.012$ \\
\textbf{J013449.35+010302.2} & $23.7057$ & $+1.0506$ & $1.2348 \pm 0.0021$ & $22.10 \pm 0.02$ & $21.73 \pm 0.02$ & $44.75 \pm 1.01$ & $3.05 \pm 0.39$ & $-0.70 \pm 0.14$ & $0.042$ \\
\textbf{J211843.66$-$002122.0} & $319.6819$ & $-0.3561$ & $1.3650 \pm 0.0023$ & $22.87 \pm 0.02$ & $22.14 \pm 0.02$ & $44.28 \pm 0.94$ & $2.99 \pm 0.16$ & $-0.52 \pm 0.09$ & $0.008$ \\
\textbf{J232147.25+001853.2} & $350.4469$ & $+0.3148$ & $1.3738 \pm 0.0021$ & $21.54 \pm 0.02$ & $21.30 \pm 0.02$ & $42.53 \pm 1.53$ & $2.01 \pm 0.52$ & $-0.69 \pm 0.11$ & $-0.025$ \\
\textbf{J234433.06$-$001123.0} & $356.1378$ & $-0.1897$ & $1.4708 \pm 0.0021$ & $19.85 \pm 0.03$ & $20.55 \pm 0.03$ & $44.52 \pm 1.16$ & $3.40 \pm 0.38$ & $-0.93 \pm 0.12$ & $0.014$ \\
\textbf{J230527.69$-$003634.5} & $346.3654$ & $-0.6096$ & $1.4904 \pm 0.0027$ & $22.97 \pm 0.03$ & $22.13 \pm 0.03$ & $45.69 \pm 1.05$ & $2.91 \pm 0.28$ & $-0.75 \pm 0.13$ & $0.024$ \\
\textbf{J022536.29$-$002029.6} & $36.4012$ & $-0.3416$ & $1.5406 \pm 0.0022$ & $22.47 \pm 0.03$ & $21.79 \pm 0.03$ & $45.16 \pm 0.97$ & $2.77 \pm 0.29$ & $-0.77 \pm 0.12$ & $0.026$ \\
\textbf{J010625.24+002206.0} & $16.6052$ & $+0.3684$ & $1.5839 \pm 0.0038$ & $23.07 \pm 0.02$ & $22.20 \pm 0.02$ & $45.05 \pm 1.00$ & $2.32 \pm 0.30$ & $-0.77 \pm 0.09$ & $0.010$ \\
\textbf{J235922.96$-$004159.2} & $359.8457$ & $-0.6998$ & $1.6251 \pm 0.0036$ & $23.29 \pm 0.02$ & $22.34 \pm 0.02$ & $44.34 \pm 0.98$ & $2.80 \pm 0.22$ & $-0.51 \pm 0.11$ & $0.014$ \\
\textbf{J001548.25+000827.1} & $3.9511$ & $+0.1409$ & $1.7119 \pm 0.0046$ & $22.05 \pm 0.04$ & $21.59 \pm 0.04$ & $44.61 \pm 1.07$ & $2.90 \pm 0.41$ & $-0.72 \pm 0.18$ & $0.065$ \\
\textbf{J022514.57+000544.9} & $36.3107$ & $+0.0958$ & $1.8321 \pm 0.0070$ & $23.02 \pm 0.02$ & $22.11 \pm 0.02$ & $44.82 \pm 1.01$ & $2.59 \pm 0.32$ & $-0.68 \pm 0.13$ & $0.027$ \\
\textbf{J024037.61$-$005637.9} & $40.1567$ & $-0.9439$ & $1.8340 \pm 0.0029$ & $21.55 \pm 0.02$ & $21.21 \pm 0.02$ & $44.21 \pm 1.15$ & $3.26 \pm 0.32$ & $-0.65 \pm 0.17$ & $0.040$ \\
\textbf{J213311.55+010356.7} & $323.2982$ & $+1.0658$ & $1.8784 \pm 0.0040$ & $22.69 \pm 0.03$ & $21.93 \pm 0.03$ & $44.58 \pm 1.08$ & $2.87 \pm 0.38$ & $-0.62 \pm 0.16$ & $0.048$ \\
\textbf{J022655.43+005555.5} & $36.7310$ & $+0.9321$ & $2.1846 \pm 0.0029$ & $23.04 \pm 0.04$ & $21.99 \pm 0.04$ & $45.56 \pm 1.27$ & $2.94 \pm 0.52$ & $-0.71 \pm 0.19$ & $0.056$ \\
\textbf{J221018.78+005652.0} & $332.5783$ & $+0.9478$ & $2.1937 \pm 0.0026$ & $23.87 \pm 0.02$ & $22.37 \pm 0.02$ & $45.64 \pm 1.28$ & $2.46 \pm 0.53$ & $-0.70 \pm 0.13$ & $0.020$ \\
\textbf{J010934.56+004820.4} & $17.3940$ & $+0.8057$ & $2.4250 \pm 0.0030$ & $22.18 \pm 0.03$ & $21.51 \pm 0.03$ & $46.10 \pm 1.17$ & $2.79 \pm 0.45$ & $-0.96 \pm 0.19$ & $0.061$ \\
\textbf{J005503.61+000902.0} & $13.7650$ & $+0.1506$ & $2.4816 \pm 0.0047$ & $23.33 \pm 0.03$ & $22.18 \pm 0.03$ & $46.11 \pm 1.17$ & $2.77 \pm 0.38$ & $-0.79 \pm 0.17$ & $0.044$ \\
\textbf{J025130.43+011231.3} & $42.8768$ & $+1.2087$ & $2.6994 \pm 0.0052$ & $23.64 \pm 0.05$ & $22.19 \pm 0.05$ & $46.74 \pm 1.19$ & $2.81 \pm 0.40$ & $-0.83 \pm 0.18$ & $0.049$ \\
\textbf{J235142.11+000653.6} & $357.9255$ & $+0.1149$ & $3.0525 \pm 0.0067$ & $24.02 \pm 0.01$ & $22.78 \pm 0.01$ & $46.67 \pm 1.77$ & $2.07 \pm 0.61$ & $-0.94 \pm 0.19$ & $-0.006$ \\
\textbf{J231444.09$-$000309.7} & $348.6837$ & $-0.0527$ & $3.4509 \pm 0.0172$ & $23.12 \pm 0.04$ & $21.59 \pm 0.04$ & $46.19 \pm 1.44$ & $2.75 \pm 0.42$ & $-0.84 \pm 0.22$ & $0.054$ \\
\hline
\end{tabular}%

==> cosmo_table.tex <==
\begin{tabular}{lccccc}
\toprule
Dataset & $H_0$\tnote{a} & $\Omega_m$ & $w_0$ & $w_a$ & $\ln \mathcal{Z}$ \\
\midrule
\multicolumn{6}{l}{\underline{\textbf{flat $\Lambda$CDM}}} \\
Pantheon+ \& SH0ES & $73.6 \pm 1.1$ & $0.334 \pm 0.018$ & $-1$ & -- & -- \\
DES-SN5YR & -- & $0.352 \pm 0.017$ & $-1$ & -- & -- \\
Planck 2018 & $67.66 \pm 0.42$ & $0.3111 \pm 0.0056$ & $-1$ & -- & -- \\
DESI DR2 & -- & $0.2975 \pm 0.0086$ & $-1$ & -- & -- \\
\textbf{SN~Ia} & \textbf{$73.53 \pm 1.01$} & \textbf{$0.33 \pm 0.02$} & \textbf{--} & \textbf{--} & \textbf{$886.6 \pm 0.1$} \\
\textbf{SN~Ia + AGN} & \textbf{$73.29 \pm 1.02$} & \textbf{$0.36 \pm 0.02$} & \textbf{--} & \textbf{--} & \textbf{$5449.1 \pm 0.2$} \\
\midrule
\multicolumn{6}{l}{\underline{\textbf{flat $w$CDM}}} \\
Pantheon+ \& SH0ES & $73.5 \pm 1.1$ & $0.309^{+0.063}_{-0.069}$ & $-0.90 \pm 0.14$ & -- & -- \\
DES-SN5YR & -- & $0.264^{+0.074}_{-0.096}$ & $-0.80^{+0.14}_{-0.16}$ & -- & -- \\
DESI DR2 & -- & $0.2969 \pm 0.0089$ & $-0.916 \pm 0.078$ & -- & -- \\
\textbf{SN~Ia} & \textbf{$73.51 \pm 1.02$} & \textbf{$0.30 \pm 0.07$} & \textbf{$-0.95 \pm 0.15$} & \textbf{--} & \textbf{$883.2 \pm 0.1$} \\
\textbf{SN~Ia + AGN} & \textbf{$73.93 \pm 1.03$} & \textbf{$0.48 \pm 0.03$} & \textbf{$-1.60 \pm 0.18$} & \textbf{--} & \textbf{$5453.1 \pm 0.2$} \\
\midrule
\multicolumn{6}{l}{\underline{\textbf{flat $w_0w_a$CDM}}} \\
Pantheon+ \& SH0ES & $73.3 \pm 1.1$ & $0.403^{+0.054}_{-0.098}$ & $-0.93 \pm 0.15$ & $-0.1^{+0.9}_{-2.0}$ & -- \\
DES-SN5YR & -- & $0.495^{+0.033}_{-0.043}$ & $-0.36^{+0.36}_{-0.30}$ & $-8.8^{+3.7}_{-4.5}$ & -- \\
DESI DR2 & -- & $0.352^{+0.041}_{-0.018}$ & $-0.48^{+0.35}_{-0.17}$ & $< -1.34$ & -- \\
\textbf{SN~Ia} & \textbf{$73.28 \pm 1.07$} & \textbf{$0.39 \pm 0.10$} & \textbf{$-0.92 \pm 0.18$} & \textbf{$-2.59 \pm 3.08$} & \textbf{$882.2 \pm 0.1$} \\
\textbf{SN~Ia + AGN} & \textbf{$72.66 \pm 1.08$} & \textbf{$0.56 \pm 0.02$} & \textbf{$-0.45 \pm 0.39$} & \textbf{$-16.73 \pm 5.44$} & \textbf{$5460.6 \pm 0.2$} \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item[a] Units: km s$^{-1}$ Mpc$^{-1}$.
\end{tablenotes}

==> hubble_priors_table.tex <==
\begin{tabular}{ll}
\hline
Parameter & Prior Distribution \\
\hline

%\multicolumn{2}{l}{\textbf{Supernovae}} \\
$M^0_{\rm SN}$ & $\mathcal{U}(-20, -18)$ \\[8pt]

%\multicolumn{2}{l}{\textbf{AGN}} \\
$M^0_{\rm AGN}$ & $\mathcal{U}(-26, -18)$ \\
$\alpha_{\rm AGN}$ & $\mathcal{U}(-20, 20)$ \\
$\beta_{\rm AGN}$ & $\mathcal{U}(-20, 20)$ \\
$\log \sigma_s$ & $\mathcal{U}(-2.2, 1.3)$ \\[8pt]

%\multicolumn{2}{l}{\textbf{Flatw0waCDM}} \\
$H_0$ & $\mathcal{U}(60, 80)$ \\
$\Omega_{m}$ & $\mathcal{U}(0, 1)$ \\
$w_0$ & $\mathcal{U}(-3, 1)$ \\
$w_a$ & $\mathcal{U}(-30, 1)$ \\[8pt]
\hline
\end{tabular}

==> multiband_priors_table.tex <==
\begin{tabular}{l l}
\toprule
Parameter & Distribution \\
\midrule
$\eta_{\sigma}$ & $\mathcal{N}(-0.5,\,1)$ \\
$\eta_{\tau}$ & $\mathcal{N}(0.5,\,0.5)$ \\

$\ln(\tau_{\rm{UV}} / {\rm days})$ & $\mathcal{TN}\!\big(\ln(10^{2.5}(1+z)),\,1.2\,\ln(10.0);0.0,\,\ln(10^4 (1+z))\big)$ \\
$\ln( \sigma_{\rm{UV}} / {\rm mag})$ & $\mathcal{N}(-0.6,\,1.0)$ \\

$m_{b, 0}$ (mag) & $\mathcal{N}(0.0,\,0.2)$ \\
 
$m_{1}$ (mag / std days) & $\mathcal{N}(0.0,\,0.1)$ \\

$\ell^{\mathrm{disk}}$ (days) & $\mathcal{TN}\!\big(10.0,\,5.0;\,0,\,\infty\big)$ \\

$\beta^{\mathrm{disk}}$ & $\mathcal{TN}\!\big(4/3,\,0.2;\,0,\,\infty\big)$ \\

$\kappa$ & $\mathcal{U}(0.0,\,1.0)$ \\

$\ln(\tau^{\mathrm{fast}} / {\rm days})$ & $\mathcal{TN}\!\big(\ln(10.0(1+z)),\, \ln 25.0;\,0.0,\, \ln(100.0(1+z))\big)$ \\

$\ln \Delta \sigma_{b, \mathrm{BLR}}$ & $\mathcal{U}(-1,\,1)$ \\

$\ln(\ell^{\mathrm{BLR}}_b / {\rm days})$ & $\mathcal{U}\!\big(\ln 2.0,\,\ln 5000.0\big)$ \\

$\ln \sigma_{\rm{jit}}$ & $\mathcal{N}\!\big(\ln\bar{\sigma}_y,\,1.0\big)$ \\
\addlinespace[0.5em]
\bottomrule
\end{tabular}


==> param_results.tex <==
% Auto-generated cosmological and evidence results
% Do not edit manually; regenerated by write_results_tex_variables()
\newcommand{\resultNumAGNPlotted}{7101}
\newcommand{\resultNumAGNFitted}{6992}
\newcommand{\resultAgeUniverse}{\ensuremath{11.26\pm0.20\,\mathrm{Gyr}}}
\newcommand{\resultPreferredModelOverall}{Flatw0waCDM}
\newcommand{\resultLogZFlatwZerowaCDM}{5460.6}
\newcommand{\resultLogZerrFlatwZerowaCDM}{0.2}
\newcommand{\resultDeltaLogZFlatwZerowaCDM}{0.0}
\newcommand{\resultSigmaFlatwZerowaCDM}{0.0}
\newcommand{\resultJeffreysStrengthFlatwZerowaCDM}{barely worth mentioning}
\newcommand{\resultLogZFlatwCDM}{5453.1}
\newcommand{\resultLogZerrFlatwCDM}{0.2}
\newcommand{\resultDeltaLogZFlatwCDM}{-7.5}
\newcommand{\resultSigmaFlatwCDM}{3.9}
\newcommand{\resultJeffreysStrengthFlatwCDM}{very strong}
\newcommand{\resultLogZFlatLambdaCDM}{5449.1}
\newcommand{\resultLogZerrFlatLambdaCDM}{0.2}
\newcommand{\resultDeltaLogZFlatLambdaCDM}{-11.5}
\newcommand{\resultSigmaFlatLambdaCDM}{4.8}
\newcommand{\resultJeffreysStrengthFlatLambdaCDM}{very strong}
\newcommand{\resultDeltaLogZFlatwZeroWaCDMFlatwCDM}{\ensuremath{7.5 \pm 0.2}}
\newcommand{\resultSigmaFlatwZeroWaCDMFlatwCDM}{3.9}
\newcommand{\resultJeffreysStrengthFlatwZeroWaCDMFlatwCDM}{very strong}
\newcommand{\resultZmcFlatwZeroWaCDMFlatwCDM}{30.3}
\newcommand{\resultDeltaLogZFlatwZeroWaCDMFlatLambdaCDM}{\ensuremath{11.5 \pm 0.2}}
\newcommand{\resultSigmaFlatwZeroWaCDMFlatLambdaCDM}{4.8}
\newcommand{\resultJeffreysStrengthFlatwZeroWaCDMFlatLambdaCDM}{very strong}
\newcommand{\resultZmcFlatwZeroWaCDMFlatLambdaCDM}{47.8}
\newcommand{\resultDeltaLogZFlatwCDMFlatLambdaCDM}{\ensuremath{4.0 \pm 0.2}}
\newcommand{\resultSigmaFlatwCDMFlatLambdaCDM}{2.8}
\newcommand{\resultJeffreysStrengthFlatwCDMFlatLambdaCDM}{Strong}
\newcommand{\resultZmcFlatwCDMFlatLambdaCDM}{16.8}
\newcommand{\resultAlphaAGN}{\ensuremath{6.3 \pm 0.16}}
\newcommand{\resultBetaAGN}{\ensuremath{-1.56 \pm 0.08}}
\newcommand{\resultSigmaUVPivot}{\ensuremath{0.2}}
\newcommand{\resultTauUVRFPivot}{\ensuremath{800}}
\newcommand{\resultOmZero}{\ensuremath{0.57 \pm 0.02}}
\newcommand{\resultwZero}{\ensuremath{-0.46 \pm 0.40}}
\newcommand{\resultwa}{-16.44 \pm 5.70}
\newcommand{\resultLIntercept}{\ensuremath{(9.3 \pm 0.4)\times 10^{44}\,\mathrm{erg\,s^{-1}}}}
\newcommand{\resultAlphaAGNL}{\ensuremath{-2.52 \pm 0.06}}
\newcommand{\resultBetaAGNL}{\ensuremath{0.62 \pm 0.033}}
\newcommand{\resultScatterHD}{\ensuremath{0.81 \pm 0.023\,\mathrm{mag}}}
\newcommand{\resultScatterL}{\ensuremath{0.322 \pm 0.009\,\mathrm{dex}}}


==> param_results_zonecut.tex <==
% Auto-generated cosmological and evidence results
% Do not edit manually; regenerated by write_results_tex_variables()
\newcommand{\resultzonecutNumAGNPlotted}{7101}
\newcommand{\resultzonecutNumAGNFitted}{5648}
\newcommand{\resultzonecutAgeUniverse}{\ensuremath{11.35\pm0.22\,\mathrm{Gyr}}}
\newcommand{\resultzonecutPreferredModelOverall}{Flatw0waCDM}
\newcommand{\resultzonecutLogZFlatwZerowaCDM}{5094.3}
\newcommand{\resultzonecutLogZerrFlatwZerowaCDM}{0.2}
\newcommand{\resultzonecutDeltaLogZFlatwZerowaCDM}{0.0}
\newcommand{\resultzonecutSigmaFlatwZerowaCDM}{0.0}
\newcommand{\resultzonecutJeffreysStrengthFlatwZerowaCDM}{barely worth mentioning}
\newcommand{\resultzonecutLogZFlatwCDM}{5087.2}
\newcommand{\resultzonecutLogZerrFlatwCDM}{0.2}
\newcommand{\resultzonecutDeltaLogZFlatwCDM}{-7.0}
\newcommand{\resultzonecutSigmaFlatwCDM}{3.8}
\newcommand{\resultzonecutJeffreysStrengthFlatwCDM}{very strong}
\newcommand{\resultzonecutLogZFlatLambdaCDM}{5084.6}
\newcommand{\resultzonecutLogZerrFlatLambdaCDM}{0.2}
\newcommand{\resultzonecutDeltaLogZFlatLambdaCDM}{-9.7}
\newcommand{\resultzonecutSigmaFlatLambdaCDM}{4.4}
\newcommand{\resultzonecutJeffreysStrengthFlatLambdaCDM}{very strong}
\newcommand{\resultzonecutDeltaLogZFlatwZeroWaCDMFlatwCDM}{\ensuremath{7.0 \pm 0.2}}
\newcommand{\resultzonecutSigmaFlatwZeroWaCDMFlatwCDM}{3.8}
\newcommand{\resultzonecutJeffreysStrengthFlatwZeroWaCDMFlatwCDM}{very strong}
\newcommand{\resultzonecutZmcFlatwZeroWaCDMFlatwCDM}{28.3}
\newcommand{\resultzonecutDeltaLogZFlatwZeroWaCDMFlatLambdaCDM}{\ensuremath{9.7 \pm 0.2}}
\newcommand{\resultzonecutSigmaFlatwZeroWaCDMFlatLambdaCDM}{4.4}
\newcommand{\resultzonecutJeffreysStrengthFlatwZeroWaCDMFlatLambdaCDM}{very strong}
\newcommand{\resultzonecutZmcFlatwZeroWaCDMFlatLambdaCDM}{40.1}
\newcommand{\resultzonecutDeltaLogZFlatwCDMFlatLambdaCDM}{\ensuremath{2.7 \pm 0.2}}
\newcommand{\resultzonecutSigmaFlatwCDMFlatLambdaCDM}{2.3}
\newcommand{\resultzonecutJeffreysStrengthFlatwCDMFlatLambdaCDM}{Strong}
\newcommand{\resultzonecutZmcFlatwCDMFlatLambdaCDM}{11.0}
\newcommand{\resultzonecutAlphaAGN}{\ensuremath{5.8 \pm 0.15}}
\newcommand{\resultzonecutBetaAGN}{\ensuremath{-1.41 \pm 0.07}}
\newcommand{\resultzonecutSigmaUVPivot}{\ensuremath{0.2}}
\newcommand{\resultzonecutTauUVRFPivot}{\ensuremath{800}}
\newcommand{\resultzonecutOmZero}{\ensuremath{0.55 \pm 0.03}}
\newcommand{\resultzonecutwZero}{\ensuremath{-0.56 \pm 0.38}}
\newcommand{\resultzonecutwa}{-13.56 \pm 5.45}
\newcommand{\resultzonecutLIntercept}{\ensuremath{(1.31 \pm 0.06)\times 10^{45}\,\mathrm{erg\,s^{-1}}}}
\newcommand{\resultzonecutAlphaAGNL}{\ensuremath{-2.3 \pm 0.06}}
\newcommand{\resultzonecutBetaAGNL}{\ensuremath{0.57 \pm 0.03}}
\newcommand{\resultzonecutScatterHD}{\ensuremath{0.59 \pm 0.021\,\mathrm{mag}}}
\newcommand{\resultzonecutScatterL}{\ensuremath{0.237 \pm 0.009\,\mathrm{dex}}}

